A Mixed Precision, Multi-GPU Design for Large-scale Top-K Sparse Eigenproblems

Graph analytics techniques based on spectral methods process extremely large sparse matrices with millions or even billions of non-zero values. Behind these algorithms lies the Top-K sparse eigenproblem, the computation of the largest eigenvalues and their associated eigenvectors. In this work, we leverage GPUs to scale the Top-K sparse eigenproblem to bigger matrices than previously achieved while also providing state-of-the-art execution times. We can transparently partition the computation across multiple GPUs, process out-of-core matrices, and tune precision and execution time using mixed-precision floating-point arithmetic. Overall, we are 67 times faster than the highly optimized ARPACK library running on a 104-thread CPU and 1.9 times than a recent FPGA hardware design. We also determine how mixed-precision floating-point arithmetic improves execution time by 50% over double-precision, and is 12 times more accurate than single-precision floating-point arithmetic.

==> figures/figure_gpu_scaling.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/gpu_scaling.pdf}
    \label{fig:gpu_scaling}
    \caption{Relative execution time for increasing number of \glspl{gpu}. 
    We observe two small outlier matrices, plotted separately, where increasing the number of \glspl{gpu} causes a performance drop due to the larger amount of inter-\gls{gpu} communication.}
\end{figure}

==> figures/figure_lanczos.tex <==
\algrenewcommand\algorithmicindent{1.2em}%
\begin{algorithm}[t]
  \caption{Top-K eigenvalues/vectors Lanczos algorithm}\label{alg:lanczos}
  \begin{algorithmic}[1]
    \Function{Lanczos}{$\mathbf{M},K,v_1$} 
    % \LineComment{\textbf{Initialization}}
    % \State $w_1 \gets \mathbf{M}v_1$ \Comment{Sparse matrix-vector multiplication}
    % \State $\alpha_1 \gets w_1 v_1$
    % \State $w'_1 \gets w_1 - \alpha_1 v_1$
    \State $\beta_1 \gets 0$ \Comment{Initialization}
    \State $v_0 \gets \textbf{0}_N$ 

    \For{$i$ in $1, K$}     \Comment{\textbf{Main Lanczos loop}}
    \LineComment{\textbf{Normalize previous Lanczos vector}}
    \If{$i > 1$}
    \State $\beta_i \gets$ $\|w'_{i - 1}\|_2$
    \State $v_i \gets w'_{i - 1} / \beta_i$ \Comment{Obtain new Lanczos vector}
    \EndIf
    \LineComment{\textbf{Begin computation of new Lanczos vector}}
    \State $w_i \gets \mathbf{M}v_i$ \Comment{Sparse matrix-vector multiplication}
    \State $\alpha_i \gets w_i v_i$
    \State $w'_i \gets w_i - \alpha_i v_{i}  - \beta_i v_{i - 1}$
    \State Orthogonalize $w'_i$ with respect to $\mathcal{V}$
    \EndFor
    \LineComment{\textbf{Tridiagonal matrix $\mathcal{T}$ and Lanczos vectors $\mathcal{V}$}}
    \State \Return $\{\mathcal{T} = [\alpha_1, \ldots, \alpha_K], [\beta_1, \ldots, \beta_{K - 1}]\}$ 
    \State \Return $\mathcal{V} = [v_1, \ldots, v_K]$
    
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> figures/figure_orthogonality.tex <==
\begin{figure}%
    \centering
     \includegraphics[width=\columnwidth]{figures/orthogonality.pdf}
    \label{fig:orthogonality}
    \caption{Accuracy of our eigensolver, in terms of average pairwise orthogonality of the extracted eigenvectors.}
\end{figure}
